Multimodal Query Suggestion with Multi-Agent Reinforcement Learning from Human Feedback

In the rapidly evolving landscape of information retrieval, search engines strive to provide more personalized and relevant results to users. Query suggestion systems play a crucial role in achieving this goal by assisting users in formulating effective queries. However, existing query suggestion systems mainly rely on textual inputs, potentially limiting user search experiences for querying images. In this paper, we introduce a novel Multimodal Query Suggestion (MMQS) task, which aims to generate query suggestions based on user query images to improve the intentionality and diversity of search results. We present the RL4Sugg framework, leveraging the power of Large Language Models (LLMs) with Multi-Agent Reinforcement Learning from Human Feedback to optimize the generation process. Through comprehensive experiments, we validate the effectiveness of RL4Sugg, demonstrating a 18% improvement compared to the best existing approach. Moreover, the MMQS has been transferred into real-world search engine products, which yield enhanced user engagement. Our research advances query suggestion systems and provides a new perspective on multimodal information retrieval.

==> method.tex <==
\section{METHODOLOGY}
\label{sec:method}


\begin{table*}[]
\centering
%\setlength{\tabcolsep}{2pt}
\caption{A running example of GPT-assisted image-suggestion labeling. Step 1: Given an image, such as a bicycle with a broken chain, the GPT model generates multiple candidate suggestions by utilizing the extracted captions from the image. Step 2: GPT-4 assigns a label (0 or 1) to each suggestion, indicating user intent, and provides a confidence score associated with the label. Step 3: Using a confidence threshold, suggestions with low confidence are filtered out and subjected to human annotation. The final labels are then produced.
}
\begin{tabular}{cl|cc|ccc}
\hline
\multicolumn{2}{c|}{Step 1}                             & \multicolumn{2}{c|}{Step 2} & \multicolumn{3}{c}{Step 3}  \\ \hline
Query Image         & \multicolumn{1}{c|}{Suggestions}  & GPT          & Conf         & Thres (0.5) & Human & Labels \\\hline
\multirow{5}{*}{\begin{minipage}[b]{0.3\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{figures/bike.JPG}}
	\end{minipage}} & How to fix a broken bicycle chain & 1            & 0.7          & \color{green}{$\surd$}    & -     & 1      \\
                    & Bicycle chain cleaning            & 1            & 0.3          & \color{red}{$\times$}   & 0     & 0      \\
                    & Bicycle brand rankings            & 0            & 0.6          & \color{green}{$\surd$}    & -     & 0      \\
                    & Nearby bicycle repair stalls      & 1            & 0.8          & \color{green}{$\surd$}    & -     & 1      \\
                    & Mountain bike prices              & 1            & 0.4          & \color{red}{$\times$}   & 0     & 0      \\ \hline
\end{tabular}
\label{tab:labeling}
\end{table*}

\subsection{Overview of \texttt{SuggGPT}}
\label{sec:overview}

The proposed solution \texttt{SuggGPT} addresses the problem of Multi-Modal Query Suggestion (MMQS) by generating intentional and diverse query suggestions based on user query images. The framework consists of several key components, including GPT-assisted image-suggestion labeling (Section~\ref{sec:data_labeling}), RewardNet training (Section~\ref{sec:reward_model}), PolicyNet training (Section~\ref{sec:policy_network}), and diversity enhancement processing (Section~\ref{sec:postprocessing}).

\underline{In the GPT-assisted labeling}, the language generation capabilities of GPT models are utilized to automate the collection of image-suggestion pairs and the annotation of user intents. This approach combines the power of automation with the reliability of manual annotation to control the quality of the prepared suggestion data for training.
%
\underline{In the RewardNet}, it is trained using annotated image-suggestion pair data and provides scores for each pair, indicating the likelihood of user interest in clicking the suggestion. To do this, a multi-task learning approach is proposed, which optimizes three pre-training tasks for the RewardNet, to enhance the training process and generate informative rewards. The output rewards represent the quality of a generated suggestion and serves as a crucial factor in the training of the PolicyNet.
%
\underline{In the PolicyNet}, it is trained using Reinforcement Learning from Human Feedback (RLHF) to generate query suggestions that align with user intent. The RLHF approach enables the model to learn from user feedback and optimize the generation of high-quality suggestions. The PolicyNet is built on top of a two-tower structure, which incorporates both visual and textual features, and further connects a Large Language Model (LLM) to enhance the model's understanding and generation capabilities. 
%
\underline{In the diversity enhancement}, it is to enhance the diversity of query suggestions within a sequence of candidate suggestions. By considering semantic similarity between the suggestions, the algorithm selects a set of distinct suggestions, providing users with a more comprehensive choices to activate the search.

We explain some insights behind the \texttt{SuggGPT} design as follows. (1) \texttt{SuggGPT} is built based on the combination of automation and manual annotation for preparing the training data. The approach simplifies the data collection process, and reduces the reliance on human annotators for RLHF. 
%
(2) The multi-task learning in RewardNet training and RLHF in PolicyNet training enable the models to learn from various tasks and user feedback, leading to improved performance in generating user intentional query suggestions.
%
(3) The diversity enhancement component selectively filters the suggestions from a pool of candidate suggestions, ensuring that the output suggestions are informative to reflect different aspects of the input query.

\subsection{Data Preprocessing}
\label{sec:data_labeling}

We investigate the utilization of GPT for assisting in image-suggestion labeling during data preprocessing. This process involves collecting image-suggestion pairs and annotating user intents regarding whether they clicked on the suggestions or not. The collected data is then utilized to train both the RewardNet and the PolicyNet models.
%
However, the process becomes time-consuming and lacks well-defined guidelines when relying on human crowd-sourcing for the data collection. Inspired by recent GPT models in various text annotation tasks~\cite{gilardi2023chatgpt,liu2023visual,OpenAI2023GPT-4}, we propose a novel approach that leverages the power of GPT-4 to automate the collection of image-suggestion pairs and annotate user intents as 0 or 1 based on potential clicks by them. This approach aims to provide a balance between automation (by GPT-4) and manual effort (by human annotators), accomplished through the implementation of a threshold-based mechanism. We illustrate a running example for the labeling in Table~\ref{tab:labeling}, and it involves the following three steps. 

\emph{Step 1: Candidate Suggestion Generation}.
%(e.g., provided by CoCo~\cite{lin2014microsoft}) or target entities (e.g., provided by ImageNet~\cite{russakovsky2015imagenet})
Leveraging extracted information from an image, such as image captions, GPT-4 initially employs its language generation capabilities to generate multiple candidate suggestions. These suggestions are designed to capture various aspects of the image, providing a wide range of options that may align with their interests.

\emph{Step 2: Labeling and Confidence Estimation}.
Once the candidate suggestions are generated, GPT-4 proceeds to label each suggestion based on its relevance to the image and potential user intent. The process enables GPT-4 to assign a binary label (e.g., 1 or 0) to each suggestion, indicating the user interest in clicking the suggestion for a given image query or not. Additionally, GPT-4 provides a confidence score (ranging between 0 and 1) associated with each label. The confidence score serves as an indicator of the model's certainty in its own labels.

\emph{Step 3: Threshold-based Annotation}.
To mitigate the reliance on manual annotation while maintaining annotation quality, we introduce a threshold-based mechanism. The confidence scores generated by GPT-4 are used to determine the level of confidence in the suggested annotations. By setting a threshold value denoted by $\alpha$, suggestions with low confidence scores are identified for further manual annotation. This approach reduces the burden of extensive manual annotation while ensuring that suggestions with lower confidence are subject to human review.

We note that the proposed labeling approach offers several innovative aspects in the field of data collection and intent annotation. First, by utilizing GPT-4's language generation capabilities, we can generate a wide range of candidate suggestions based on image content, providing a comprehensive set of options for users. Second, the labeling and confidence estimation step enhances the reliability of the generated suggestions by quantifying the model's confidence. Third, the threshold-based mechanism introduces a customizable parameter, which facilitates the workload adjustment between automation and human effort according to specific requirements.

\begin{figure*}
  \centering
  \includegraphics[width=0.75\textwidth]{figures/SuggGPT-3.drawio.pdf}
  \caption{Illustration of RewardNet and PolicyNet. In RewardNet, it is optimized using multi-task learning (ISA, ISG, and ISM), and employs learnable query embeddings to capture visual representations. In PolicyNet, it also follows a two-tower structure, and generates final query suggestions that are optimized for intentionality through IE and diversity through DE.}\label{fig:overall}
\end{figure*}

\subsection{RewardNet Training}
\label{sec:reward_model}
In this section, we introduce the training process of the RewardNet, utilizing the annotated image-suggestion pair data. The RewardNet provides scores (e.g., a value ranging between 0 and 1) for each image-suggestion pair, indicating the likelihood of user interest in clicking the suggestion for a given image query. Below, we present the model architecture and training details for the RewardNet.

\smallskip
\noindent \textbf{Model Architecture.} As shown in Figure~\ref{fig:overall}, our proposed RewardNet comprises two transformer-based modules, namely Image-Tower and Text-Tower, which share common self-attention layers to capture both visual and textual features. 
%
For the Image-Tower, it is responsible for interacting with a pre-trained frozen image encoder to extract visual features. To achieve this, we introduce a set of learnable query embeddings as input to the Image-Tower. These queries interact with each other through self-attention layers, and also with the frozen image features through cross-attention layers, which are inserted alternately in the Image-Tower blocks. 
%
For the Text-Tower, we enable textual suggestions to engage with the learnable query embeddings by leveraging shared self-attention layers. To boost the training efficiency, we initialize the self-attention layers and feed-forward layers with pre-trained weights from BERT~\cite{kenton2019bert}, and the cross-attention layers are randomly initialized.

\smallskip
\noindent \textbf{RewardNet Training.} We explore a multi-task learning for the RewardNet, leveraging the joint optimization of three pre-training tasks, namely Image-Suggestion Alignment (ISA), Image-Suggestion Generation (ISG), and Image-Suggestion Matching (ISM). The rationale behind the design is to effectively enhance the training process of the RewardNet, ensuring the generation of informative rewards guided by these typical tasks. 

In ISA, the objective is to align image representation and suggestion representation such that the model projects similar images and suggestions closer in the embedding space while pushing unrelated pairs further apart. To achieve this, it creates a contrast by comparing the image-suggestion similarity of a positive pair to that of negative pairs. Specifically, we sample a batch of image-suggestion pairs denoted by $\mathcal{V}$, where each pair consists of an image and its corresponding suggestion, annotated with the label 1. Then, for each pair $<I_i, S_i> \in \mathcal{V}$, we denote its vector representations as $<\mathbf{v}_i^{I}$ and $\mathbf{v}_i^{S}>$ ($1 \le i \le n$), where $n$ denotes the batch size. 
%
We consider $\mathbf{v}_i^{S}$ as the positive of $\mathbf{v}_i^{I}$, and the negatives as the other suggestions in the same batch. Then, the contrastive loss is formulated as 

\begin{align}
    \label{eq:clLoss}
    \mathcal{L}_\text{ISA} = \sum\nolimits_{<I_i, S_i> \in \mathcal{V}} -\log \frac{\exp\Bigm({\mathbf{v}_i^{I}\cdot\mathbf{v}_i^{S}/\tau}\Bigm)}{ \sum\nolimits_{<I_j, S_j> \in \mathcal{V}, j\neq i} \exp\Bigm({\mathbf{v}_i^{I}\cdot\mathbf{v}_j^{S}/\tau}\Bigm)},
\end{align}
where $\tau$ represents a temperature parameter in contrastive learning. 

In ISG, the objective is to generate suggestions based on the underlying image content, thereby enhancing the RewardNet's ability to accurately assign scores to image-suggestion pairs. This is achieved by ensuring that the generated suggestions are semantically consistent with the visual context of the grounded image. Specifically, given an image-suggestion $<I, S>$ pair, where the suggestion $S$ corresponds to a sequence of word tokens $S = <w_1, ..., w_m>$, we employ a language generation loss to maximize the conditional probability $P$ as follows:

\begin{align}
    \label{eq:glLoss}
    \mathcal{L}_\text{ISG} = \sum\nolimits_{i} \log P(w_i|w_{1:i-1},I).
\end{align}

In ISM, the objective is to establish a precise alignment between image and suggestion representations through fine-grained learning. This involves a binary classification task in which the model is to predict whether an image-suggestion pair is positive (matched) or
negative (unmatched). To achieve this, we employ a hard negative mining strategy, where hard negative samples are defined as candidate suggestions of an image annotated with the label 0. The rationale behind this strategy is that while some suggestions are related to the query image, they fail to capture the user's search intent. By optimizing with these hard samples, the RewardNet is encouraged to assign high scores to image-suggestion pairs exhibiting a strong correlation between the image and text representations. Then, the objective is trained using a binary cross-entropy loss, formulated as follows:

\begin{align}
    \label{eq:mlLoss}
    \mathcal{L}_\text{ISM} = - (y * \log(P) + (1 - y) * \log(1 - P)),
\end{align}
where $y$ denotes the true label (either 0 or 1), and $P$ is the predicted probability of the positive class.

Finally, the RewardNet is trained using a multi-task learning approach, where the loss function $\mathcal{L}_\text{RN}$ is defined as follows:

\begin{align}
    \label{eq:Loss}
    \mathcal{L}_\text{RN} = \mathcal{L}_\text{ISA} + \mathcal{L}_\text{ISG} + \mathcal{L}_\text{ISM}.
\end{align} 
The reward is then defined as the predicted probability $P$ in the Image-Suggestion Matching task, because it represents a normalized value ranging from 0 to 1, which avoids potential data scale issues that may arise during the training process, that is

\begin{align}
    \label{eq:reward}
    r_{\theta}(I,S) = P,
\end{align} 
where $r_{\theta}(I,S)$ represents the reward output of the RewardNet for a given query image $I$ and its associated suggestions $S$, with parameters denoted as $\theta$.

\subsection{PolicyNet Training}
\label{sec:policy_network}
The objective of MMQS is to generate query suggestions that align with users' intended search queries, specifically those that are more likely to be clicked. This motivates us to explore the application of Reinforcement Learning from Human Feedback (RLHF) technique in training the PolicyNet. Below, we present the model architecture, RLHF modeling, and training details for the RewardNet.

\smallskip
\noindent \textbf{Model Architecture.} In PolicyNet, we adopt a similar two-tower structure as presented in the RewardNet, to capture both visual and textual features. Additionally, we aim to leverage the language generation capability of a LLM by establishing a connection between the Image-Tower and the LLM. As shown in Figure~\ref{fig:overall}, the connection is implemented using a fully-connected (FC) layer. The FC layer projects the output query embeddings to align with the dimensionality of the LLM's text embedding, and then these projected query embeddings are concatenated at the beginning of the input text embeddings. This integration serves the visual information as soft prompts, conditioning the LLM on the visual representations to generate language. Notably, the LLM is kept frozen during training to facilitate the process.

\smallskip
\noindent \textbf{RLHF Modeling.} We model the suggestion generation with RLHF, involving states, actions, and rewards. 

\emph{States}: The state $s$ is defined by the query embeddings of an input query image, which undergoes a process to extract the representation. Specifically, the image is first encoded using a frozen Vision Transformer (ViT)~\cite{radford2021learning}, which produces a fixed-length representation of the image that captures its visual features. Then, some learnable query embeddings are generated as the design in RewardNet, these embeddings represent the different aspects of the query image that the model should attend to, and the query embeddings are then passed through cross-attention layers, which allow them to interact with the frozen visual features. By leveraging this approach, we can effectively incorporate the contextual relationships between the queries and the image features, and forming a comprehensive representation of the state.

\emph{actions}: The action $a$ is defined by the generated suggestions via a LLM, which conditions on the state visual representations to generate language. Here, We employ a decoder-only language model (e.g., OPT~\cite{zhang2022opt}) for its simplicity and efficiency, as it does not require encoding visual information, and only to generate suggestions that are relevant to the image. This enables our training more efficiently and reduces the GPU requirements.

\emph{rewards}: According to Equation~\ref{eq:reward}, the reward is represented by $r_{\theta}(s,a)$, which is obtained from the RewardNet. The purpose of training the reward model is to accurately predict the quality of a generated suggestion, as assessed by human judgment, for a given query image. This enables us to optimize the generation of high-quality suggestions that align with human preferences.

\smallskip
\noindent \textbf{PolicyNet Training.} We discuss the learning process of PolicyNet, which involves a two-stage training: Supervised Fine-Tuning (SFT) stage and Proximal Policy Optimization (PPO) stage.

For SFT stage, it provides a necessary warm-start before the policy training, which equips the LLM with the abilities to generate suggestions. Specifically, in this stage, the PolicyNet undergoes a two-step process. Firstly, the two towers are trained using a multi-task learning approach (ISA, ISG, and ISM) according to Equation~\ref{eq:mlLoss}. This approach allows the two towers to learn from different related tasks simultaneously, enhancing the representations of both images and suggestions, where the two towers leverage the shared knowledge from the tasks and improve its understanding of the underlying data. Subsequently, the connection between the LLM and the visual representations is fine-tuned using a language generation loss according to Equation~\ref{eq:glLoss}. By conditioning the LLM on the visual representations, it can capture the visual cues presented in the input image, enabling the generation of suggestions that align effectively with the image content. 

For PPO stage, we utilize the PPO algorithm~\cite{schulman2017proximal} to fine-tune the SFT model for our specific environment. Our environment is designed as a bandit setting, where a random query image is presented, and the model generates a suggestion in response to the image, and ends the episode. Following the suggestion generation, the environment calculates a reward based on the evaluation of RewardNet. To prevent over-optimization of the RewardNet, we further incorporate a penalty for the KL divergence~\cite{jaques2019way} between the learned RL policy, denoted as $\pi_{\phi}^{\text{RL}}$ with parameters $\phi$, and its original SFT policy, denoted as $\pi^\text{SFT}$.

\begin{align}
    \label{eq:policy}
    \mathcal{L}_\text{PN} = r_{\theta}(s,a) - \beta\log(\pi_{\phi}^{\text{RL}}(a|s)/\pi^{\text{SFT}}(a|s)),
\end{align} 
where $\beta$ represents a KL reward coefficient, which controls the strength of the penalty.

\subsection{Diversity Enhancement}
\label{sec:postprocessing}

\begin{algorithm}[t!]
	\caption{Diversity Enhancement Algorithm}
	\label{alg:diversity}
		\KwIn{
		a sequence of candidate suggestions $<S_1, S_2, ... >$; a parameter $K$; a threshold parameter $\delta$}
        \For{$i=1,2,...$}{
			\uIf{$i=1$}{
			$\mathcal{S} \leftarrow S_1$;
            }
           \uElse{
            \For{$j=1,2,...,|\mathcal{S}|$}{
            calculate the semantic similarity between $S_i$ and $\mathcal{S}[j]$, and maintain the maximum similarity, denoted by $\delta'$;
            }
            \uIf{$\delta' < \delta$}{
			$\mathcal{S} \leftarrow S_i$;
            }
            }
     
        \uIf{$|\mathcal{S}| = K$}{
        \textbf{Break};
        }
}
\textbf{Return} $\mathcal{S}$;
\end{algorithm}

In this section, we propose an algorithm designed to address the diversity property discussed in Section~\ref{sec:problem}. The primary objective of this algorithm is to enhance the overall variety of suggestions and provide users with a more comprehensive selection.
%
The idea behind the algorithm is to promote diversity within a sequence of candidate suggestions, which can be obtained via the proposed \texttt{SuggGPT} from different application scenarios (e.g., generation-based search engine or retrieval-based search engine), as we will discuss later. 
%
Further, by incorporating a threshold parameter $\delta$ for semantic similarity (e.g., measuring via BERT~\cite{kenton2019bert}) and a Top-$K$ parameter for specifying the desired number of diverse suggestions, the algorithm can select a set of suggestions that are distinct from each other.

Specifically, the process is presented in Algorithm~\ref{alg:diversity}, it takes three parameters as the input: a sequence of candidate suggestions denoted as $<S_1, S_2, ...>$, Top-$K$, and the threshold $\delta$.
%
The algorithm iterates through the candidate suggestions in the input sequence (lines 1-12). The first suggestion $S_1$ is assigned to the set $\mathcal{S}$ (lines 2-3). In the subsequent iterations, it calculates the semantic similarity between the current suggestion $S_i$ and each suggestion in the set $\mathcal{S}$, maintaining the maximum similarity value denoted as $\delta'$ (lines 4-7). This step ensures that only the most similar suggestion in $\mathcal{S}$ to $S_i$ is considered.
%
If the maximum similarity $\delta'$ is below the threshold $\delta$, indicating that the current suggestion $S_i$ is sufficiently dissimilar to all suggestions in $\mathcal{S}$, then $S_i$ is inserted into $\mathcal{S}$ (lines 8-9)
%
The algorithm continues until the size of $\mathcal{S}$ reaches the desired diversity parameter $K$ (lines 10-11). At this point, the algorithm terminates, and the set $\mathcal{S}$ containing $K$ diverse suggestions is returned (line 13).


\subsection{Discussion on Applications and Cold-start Problem}

\noindent \textbf{Supporting Generation-based and Retrieval-based Applications.} We discuss the capabilities of \texttt{SuggGPT} to support two application scenarios in search engines: generation-based and retrieval-based. 
%
In the generation-based scenario, \texttt{SuggGPT} utilizes its language generation capability from large language models (LLMs) to generate query suggestions in response to users' image queries across a wide range of domains. 

In the retrieval-based scenario, \texttt{SuggGPT} specializes in providing query suggestions for specific domains with narrower focuses, such as commodities, animals, or plants, where the suggestions can be prepared in advance. Specifically, \texttt{SuggGPT} leverages its ability to represent both language and images. It preprocesses domain-specific images to generate targeted query suggestions, which are then stored as vector representations via the Text-Tower in a database. To facilitate search efficiency, a vector index, such as HNSW, can be incorporated. During the inference stage, \texttt{SuggGPT}'s image encoder extracts the representation of a user's input image, and a nearest neighbor search is conducted within the suggestion database. This process retrieves the Top-$K$ query suggestions that exhibit the highest similarity to the user's input image. This application offers several advantages. Firstly, vector-based retrieval is known for its efficiency to response users' queries. Additionally, by precomputing and storing the query suggestions in a database, the reliability of these suggestions can be ensured in advance, resulting in a more friendly user experience.

\smallskip
\noindent \textbf{Handling the Cold-start Problem.} As \texttt{SuggGPT} relies on feedback from labelers to capture search intentionality, there is a potential cold-start problem in generating recommended suggestions when the learned knowledge may not be sufficient for certain user queries. To address this issue, we implement an online learning strategy for \texttt{SuggGPT}, involving continuous fine-tuning of both the RewardNet and the PolicyNet using newly recorded query images and users' click behaviors for the suggestions. This strategy ensures that the model's policy remains updated for online applications. We have validated the effectiveness of this strategy in Section~\ref{sec:effectiveness}, and the results demonstrate that the deployed system incorporating this strategy significantly enhances the user experience. For example, we observe a notable increase in click behaviors by {\Comment 0.31\%}, highlighting the positive impact of this strategy.

\label{sec:application}

==> method2.tex <==
\section{METHODOLOGY}
\label{sec:method}

\subsection{Overview of \texttt{RL4Sugg}}
\label{sec:overview}

The proposed solution \texttt{RL4Sugg} addresses the problem of Multimodal Query Suggestion (MMQS) by generating intentional and diverse query suggestions based on user query images. The framework consists of several key components, including data preparing (Section~\ref{sec:data_labeling}), RewardNet training (Section~\ref{sec:reward_model}), and PolicyNet training (Section~\ref{sec:policy_network}).

\underline{In data preparing}, the language generation capabilities of LLMs are utilized to automate the collection of image-suggestion pairs and the annotation of user intents. This approach combines the power of automation with the reliability of manual annotation to control the quality of the prepared suggestion data for training.
%
\underline{In RewardNet training}, it is trained using annotated image-suggestion pair data and provides scores (rewards) for each pair, indicating the likelihood of user interest in clicking the suggestion. To do this, a multi-task learning approach is proposed, which optimizes three pre-training tasks for the RewardNet, to enhance the training process and generate informative rewards. The output rewards represent the quality of a generated suggestion and serves as a crucial factor in the training of the PolicyNet.
%
\underline{In PolicyNet training}, the PolicyNet utilizes a two-tower structure to capture visual and textual features and incorporates a LLM to enhance understanding and generation capabilities. It is trained using RLHF to generate query suggestions that align with user intent, learning from user feedback for high-quality suggestions. Additionally, we include a diversity loss in the RLHF training, enabling the model to optimize both intentionality and diversity of the generated suggestions in an end-to-end manner.

We explain some insights behind the \texttt{RL4Sugg} design as follows. (1) \texttt{RL4Sugg} is built based on the combination of LLM automation and human annotation for preparing the training data. The approach simplifies the data collection process, and reduces the reliance on human annotators for RLHF. 
%
(2) The multi-task learning in RewardNet training and RLHF in PolicyNet training enable the models to learn from various tasks and user feedback, leading to improved performance in generating user intentional suggestions.
%
(3) The diversity loss is trained to minimize the similarity between generated suggestions, ensuring that the output suggestions are informative and reflect various aspects of the input query image.

\subsection{Data Preparing}
\label{sec:data_labeling}

This process involves collecting image-suggestion pairs and annotating user intents regarding their likelihood to click on the suggestions or not. However, relying solely on human crowd-sourcing for data collection can be time-consuming and lack clear guidelines. To address this, inspired by language generation capabilities from recent GPT models~\cite{gilardi2023chatgpt,liu2023visual,OpenAI2023GPT-4}, we propose a novel approach using GPT-4 to automate image-suggestion pair collection and user intent annotation based on potential clicks. This approach provides a balance between automation (by GPT-4) and manual effort (by human annotators) through a threshold-based mechanism. To better illustrate the labeling process, we present a running example in Table~\ref{tab:labeling}, which involves three key steps.

\emph{Step 1: Candidate Suggestion Generation}.
Leveraging extracted information (e.g., captions) from an image, GPT-4 initially employs its language generation capabilities to generate multiple candidate suggestions. These suggestions are designed to capture various aspects of the image, providing a wide range of options that may align with their interests.

\emph{Step 2: Labeling and Confidence Estimation}.
Once the candidate suggestions are generated, GPT-4 further proceeds to label each suggestion based on its relevance to the image and potential user intent. The process enables GPT-4 to assign a binary label (i.e., 1 or 0) to each suggestion, indicating the user interest in clicking the suggestion for a given query image or not. In addition, GPT-4 provides a confidence score (ranging between 0 and 1) associated with each label, which serves as an indicator of the model's certainty in its own labels.

\emph{Step 3: Threshold-based Annotation}.
To mitigate the reliance on manual annotation while maintaining annotation quality, we introduce a threshold-based mechanism. The confidence scores generated by GPT-4 are used to indicate the quality of the suggested annotations. By setting a threshold value, suggestions with low confidence scores are identified for further manual annotation. This approach reduces the burden of extensive manual annotation while ensuring that suggestions with lower confidence are subject to human review.

We note that the proposed labeling approach offers several innovative aspects in the field of text annotation tasks~\cite{gilardi2023chatgpt,liu2023visual,OpenAI2023GPT-4}. First, by utilizing GPT-4's language generation capabilities, we can generate a wide range of candidate suggestions based on image content, providing a comprehensive set of options for users. Second, the labeling and confidence estimation step enhances the reliability of the generated suggestions by quantifying the model's confidence. Third, the threshold-based mechanism introduces a customizable parameter, which facilitates the workload adjustment between automation and human effort according to specific requirements.

\begin{figure*}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/SuggGPT-5.drawio.pdf}
  \caption{Illustration of RewardNet and PolicyNet. In RewardNet, it is trained with multi-task learning (ISA, ISG, and ISM), where learnable query embeddings are employed to extract visual representations from different aspects, and align the textual suggestion (whose representation is captured by the $[CLS]$ token) with the most relevant one. In PolicyNet, it follows a two-tower structure, and generates final query suggestions that are optimized for intentionality through IE and diversity through DE.}\label{fig:overall}
\end{figure*}

\subsection{RewardNet Training}
\label{sec:reward_model}
In this section, we introduce the training process of the RewardNet, utilizing the annotated image-suggestion pair data. The RewardNet provides rewards (e.g., a value ranging between 0 and 1) for each image-suggestion pair, indicating the likelihood of user interest in clicking the suggestion for a given query image. Below, we present the model architecture and training details for the RewardNet.

\smallskip
\noindent \textbf{Model Architecture.} As shown in Figure~\ref{fig:overall}, our proposed RewardNet follows a two-tower structure incorporating two transformer-based modules, namely Image-Tower and Text-Tower, which share common self-attention layers to capture both visual and textual features. 
%
In the Image-Tower, it is responsible for interacting with a pre-trained frozen image encoder to extract visual features. To achieve this, we introduce a set of learnable query embeddings as input to the Image-Tower. These queries interact with each other through self-attention layers, and also with the frozen image features through cross-attention layers, which are inserted alternately in the Image-Tower blocks. 
%
In the Text-Tower, we enable textual suggestions to engage with the learnable query embeddings by leveraging shared self-attention layers. To boost the training efficiency, we initialize the self-attention layers and feed-forward layers with the pre-trained weights from BERT~\cite{kenton2019bert}, and the cross-attention layers are randomly initialized.

\smallskip
\noindent \textbf{Training Paradigm.} We explore a multi-task learning for the RewardNet, leveraging the joint optimization of three pre-training tasks, namely Image-Suggestion Alignment (ISA), Image-Suggestion Generation (ISG), and Image-Suggestion Matching (ISM). The rationale behind the design is to effectively enhance the training process of the RewardNet, ensuring the generation of informative rewards guided by these typical tasks. 

In ISA, the objective is to align image representation and suggestion representation such that the model projects similar images and suggestions closer in the embedding space while pushing unrelated pairs further apart. To achieve this, it creates a contrast by comparing the image-suggestion similarity of a positive pair to that of negative pairs. Specifically, we sample a batch of image-suggestion pairs denoted by $\mathcal{V}$, where each pair consists of an image and its corresponding suggestion, annotated with the label 1. Then, for each pair $<I_i, S_i> \in \mathcal{V}$, we denote its vector representations as $\mathbf{V}_i^{I}$ and $\mathbf{v}_i^{S}$ ($1 \le i \le n$), where $n$ denotes the batch size, $\mathbf{V}_i^{I}$ is the learned query embeddings from Image-Tower, and $\mathbf{v}_i^{S}$ is the output embedding of the $[CLS]$ token from Text-Tower.
%
We consider $\mathbf{v}_i^{S}$ as the positive of $\mathbf{V}_i^{I}$ because the image $I_i$ and the suggestion $S_i$ are matched with the label 1, and the negatives as the other suggestions in the same batch. Then, the contrastive loss is defined as 

\begin{align}
    \label{eq:clLoss}
    \mathcal{L}_\text{ISA} = \sum\limits_{<I_i, S_i> \in \mathcal{V}} -\log \frac{\exp\Bigm({\max\limits_{\mathbf{v}_i^{I} \in \mathbf{V}_i^{I}}\mathbf{v}_i^{I}\cdot\mathbf{v}_i^{S}/\tau}\Bigm)}{ \sum\limits_{<I_j, S_j> \in \mathcal{V}, j\neq i} \exp\Bigm({\max\limits_{\mathbf{v}_i^{I} \in \mathbf{V}_i^{I}}\mathbf{v}_i^{I}\cdot\mathbf{v}_j^{S}/\tau}\Bigm)},
\end{align}
where $\tau$ represents a temperature parameter in contrastive learning. To determine the image-text similarity, we compute the pairwise similarity between each query embedding $\mathbf{v}_i^{I} \in \mathbf{V}_i^{I}$ and $\mathbf{v}_i^{S}$, and select the highest similarity value.

In ISG, the objective is to generate suggestions based on the underlying image content, thereby enhancing the RewardNet's ability to accurately assign scores to image-suggestion pairs. This is achieved by ensuring that the generated suggestions are semantically consistent with the visual context of the grounded image. Specifically, given an image-suggestion $<I, S>$ pair, where the suggestion $S$ corresponds to a sequence of word tokens $S = <w_1, ..., w_m>$, we employ a language generation loss to maximize the conditional probability $P$ as

\begin{align}
    \label{eq:glLoss}
    \mathcal{L}_\text{ISG} = \sum\limits_{i} -\log P(w_i|w_{1:i-1},I).
\end{align}

In ISM, the objective is to establish a precise alignment between image and suggestion representations through fine-grained learning. This involves a binary classification task in which the model is to predict whether an image-suggestion pair is positive (matched) or
negative (unmatched). To achieve this, we study a hard negative mining strategy, where hard negative samples are defined as candidate suggestions of an image annotated with the label 0. The rationale behind this strategy is that while some suggestions are related to the query image, they fail to capture the user's search intent. By optimizing with these hard samples, the RewardNet is encouraged to assign high scores to image-suggestion pairs exhibiting a strong intention between the image and text representations. Then, the objective is trained using a binary cross-entropy loss, formulated as 

\begin{align}
    \label{eq:mlLoss}
    \mathcal{L}_\text{ISM} = - y * \log(P) + (y - 1) * \log(1 - P),
\end{align}
where $y$ denotes the true label (either 0 or 1), and $P$ is the predicted probability of the positive class.

Finally, the RewardNet is trained using a multi-task learning approach, where the loss function $\mathcal{L}_\text{RN}$ is defined as

\begin{align}
    \label{eq:Loss}
    \mathcal{L}_\text{RN} = \mathcal{L}_\text{ISA} + \mathcal{L}_\text{ISG} + \mathcal{L}_\text{ISM}.
\end{align} 
The reward is then defined as the predicted probability $P$ in the Image-Suggestion Matching (ISM) task, because it represents a normalized value ranging from 0 to 1, which avoids potential data scale issues that may arise during the training process, that is

\begin{align}
    \label{eq:reward}
    r_{\theta}(I,S) = P,
\end{align} 
where $r_{\theta}(I,S)$ represents the reward outputted by the RewardNet for a given query image $I$ and its associated suggestions $S$, and $\theta$ denotes the network parameters.

\subsection{PolicyNet Training}
\label{sec:policy_network}
The objective of MMQS is to generate query suggestions that align with users' intended search queries, specifically those that are more likely to be clicked. This motivates us to explore the application of Reinforcement Learning from Human Feedback (RLHF) technique in training the PolicyNet. Further, we investigate a diversity enhancement loss into the RLHF training, which makes our model can be trained end-to-end to optimize the two query suggestion properties, i.e., intentionality and diversity. Below, we present the model architecture, and detailed designs in the PolicyNet.

\smallskip
\noindent \textbf{Model Architecture.} %We adopt a two-tower structure combined with a LLM to generate query suggestions, as illustrated in Figure~\ref{fig:overall}. The Image-Tower extracts visual features of the query image using learnable query embeddings, while the Text-Tower takes a hard prompt (e.g., a sentence) and produces its soft prompt (e.g., an embedding) to signal the LLM in generating diverse suggestions. To enable language generation, we establish a connection between the output embedding from the two-tower and the LLM, achieved through a fully-connected (FC) layer that aligns the dimensions of the output embedding with the LLM's text embedding. This projected embedding is concatenated with the input text embeddings, conditioning the LLM on the prompt to generate language. Notably, the LLM remains frozen during training to facilitate the process.
In PolicyNet, we adopt a similar two-tower structure as presented in the RewardNet, to capture both visual and textual features. Additionally, we aim to leverage the language generation capability of a LLM by establishing a connection between the Image-Tower and the LLM. As shown in Figure~\ref{fig:overall}, the connection is implemented using a fully-connected (FC) layer. The FC layer projects the output query embeddings to align with the dimensionality of the LLM's text embedding, and then these projected query embeddings are concatenated at the beginning of the input text embeddings of the LLM. This integration serves the visual information as soft prompts, conditioning the LLM on the visual representations to generate language. Notably, the LLM is kept frozen during training to facilitate the process.

\smallskip
\noindent \textbf{Intentionality Enhancement (IE).} To enhance the intentionality of the generated suggestions, we model the process with RLHF, involving states, actions, and rewards. 

\emph{States}: %The state $s$ is derived from the output embedding of the two-tower through the following process. Initially, the image is encoded using a frozen Vision Transformer (ViT)~\cite{radford2021learning}, resulting in a fixed-length representation that captures the image's visual features. Next, learnable query embeddings are generated, representing different aspects of the query image for model attention, and are passed through cross-attention layers to interact with the frozen visual features. To enhance suggestion diversity, a text-tower is introduced, taking a sentence as a hard prompt (e.g., "please output diverse query suggestions") and generating its soft prompt embedding. Finally, the state is created by fusing the query embedding and prompt embedding through self-attention.
The state $s$ is defined by the query embeddings of an input query image, which undergoes a process to extract the representation. Specifically, the image is first encoded using a frozen Vision Transformer (ViT)~\cite{radford2021learning}, which produces a fixed-length representation of the image that captures its visual features. Then, some learnable query embeddings are generated as the design in RewardNet, these embeddings represent the different aspects of the query image that the model should attend to, and the query embeddings are then passed through cross-attention layers, which allow them to interact with the frozen visual features. By leveraging this approach, we can effectively incorporate the contextual relationships between the queries and the image features, and forming a comprehensive representation of the state.

\emph{actions}: The action $a$ is defined by the generated suggestions via a LLM, which conditions on the state representation to generate language. Here, We employ a decoder-only language model (e.g., OPT~\cite{zhang2022opt}) for its simplicity and efficiency, as it does not require encoding input information, and only to generate suggestions that are relevant to the image. This enables our training more efficiently and reduces GPU requirements.

\emph{rewards}: According to Equation~\ref{eq:reward}, the reward is represented by $r_{\theta}(s,a)$, which is obtained from the RewardNet. The purpose of training the reward model is to accurately predict the quality of a generated suggestion, as assessed by human judgment, for a given query image. This enables us to optimize the generation of high-quality suggestions that align with human preferences.

\smallskip
\noindent \textbf{Diversity Enhancement (DE).} We further introduce a diversity enhancement module to augment the overall variety of suggestions and offer users a more comprehensive selection. One intuitive idea for diversity enhancement is to apply some post-processing operations, such as clustering, which groups similar suggestions into one cluster, and then selects the clustering centers as the output suggestions, resulting in a reduction of redundancy suggestions. However, these post-processing approaches encounter a challenge as language models cannot directly generate the diverse query suggestions, which makes further optimization difficult. To tackle this issue, we include diversity as one of the training objectives for PolicyNet, where we pairwise calculate semantic similarity (e.g., using BERT~\cite{kenton2019bert}) between the suggestions, and the average similarity is used to represent the diversity, which is then integrated with the RLHF during the training of the PolicyNet. This end-to-end optimization of the LLM enables the generation of suggestions that demonstrate both intentionality and diversity. 

\smallskip
\noindent \textbf{Training Paradigm.} We discuss the learning process of PolicyNet, which involves two stages: warm-start stage and training stage.

For the warm-start stage, we study the Supervised Fine-Tuning (SFT), which equips the LLM with the basic abilities to generate suggestions. Specifically, in this stage, the PolicyNet undergoes a two-step process. Firstly, the two towers are trained using a multi-task learning approach (ISA, ISG, and ISM) according to Equation~\ref{eq:mlLoss}. This approach allows the two towers to learn from different related tasks simultaneously, enhancing the representations of both images and suggestions, where the two towers leverage the shared knowledge from the tasks and improve its understanding of the underlying data. Subsequently, the connection (i.e., the FC layer) between the LLM and the two-tower is fine-tuned using a language generation loss according to Equation~\ref{eq:glLoss}. By conditioning the LLM on the output from the two-tower, it can capture the visual cues presented in the input image, enabling the generation of suggestions that align effectively with the image content. 

For the training stage, we utilize the PPO algorithm~\cite{schulman2017proximal} to fine-tune the SFT model for achieving the Intentionality Enhancement (IE) in our specific query suggestion environment, where the environment is modeled as a bandit setting, i.e., when a random query image is presented, the model generates a suggestion in response to the image, and ends the episode. Following the suggestion generation, the environment calculates a reward based on the evaluation by RewardNet. To prevent over-optimization of the RewardNet, we further incorporate a penalty for the KL divergence~\cite{jaques2019way} between the learned RL policy, denoted as $\pi_{\phi}^{\text{RL}}$ with parameters $\phi$, and its original SFT policy, denoted as $\pi^\text{SFT}$. Then, the intentionality enhancement $\mathcal{L}_\text{IE}$ loss is formulated as

\begin{align}
    \label{eq:ie}
    \mathcal{L}_\text{IE} = -r_{\theta}(s,a) + \beta\log(\pi_{\phi}^{\text{RL}}(a|s)/\pi^{\text{SFT}}(a|s)),
\end{align} 
where $\beta$ represents a KL reward coefficient, which controls the strength of the penalty. Further, we achieve the Diversity Enhancement (DE) loss $\mathcal{L}_\text{DE}$ as the average similarity of the generated suggestions $<S_1, S_2, ..., S_K>$, which is formulated as

\begin{align}
    \label{eq:de}
    \mathcal{L}_\text{DE} = \frac{\sum\nolimits_{1 \le i < j \le K} \sigma(S_i,S_j)}{K * (K-1)/2},
\end{align} 
where $\sigma(\cdot,\cdot)$ denotes the semantic similarity between two suggestions. Finally, the loss for training the PolicyNet $\mathcal{L}_\text{PN}$ is defined as 
\begin{align}
    \label{eq:policy}
    \mathcal{L}_\text{PN} = \mathcal{L}_\text{IE} + \mathcal{L}_\text{DE}.
\end{align} 



\subsection{Discussion on Applications and Cold-start Problem}
\label{sec:apps}

\noindent \textbf{Supporting Generation-based and Retrieval-based Applications.} We discuss the capabilities of \texttt{RL4Sugg} to support two application scenarios in search engines: generation-based and retrieval-based. 
%
In the generation-based scenario, \texttt{RL4Sugg} can naturally utilize its language generation capability from LLMs to generate query suggestions in response to users' image queries across a wide range of domains. 

In the retrieval-based scenario, \texttt{RL4Sugg} specializes in providing query suggestions for specific domains with narrower focuses, such as commodities for certain E-commerce shopping websites, where the query suggestions are limited to their commodities, and can be prepared in advance. Specifically, \texttt{RL4Sugg} leverages its ability to represent both images (e.g., learned query embeddings) and language (e.g., the $[CLS]$ token embedding) from the two-tower in PolicyNet. It first prepares the query suggestions for their commodities, which are then stored as vector representations into a database. To facilitate search efficiency, a vector index structure, such as HNSW, may also be incorporated. During the inference, \texttt{RL4Sugg}'s image encoder extracts the representation of a user's input image, and the nearest neighbor search can be conducted within the database, to retrieve Top-$K$ query suggestions that exhibit the highest similarity to the user's input image. We note that our \texttt{RL4Sugg} offers several advantages for this application. Firstly, the vector-based retrieval is known for its efficiency in responding to users' queries. Moreover, by precomputing and storing the query suggestions in a database, the reliability of these suggestions can be guaranteed in advance, leading to an improved user experience.

\smallskip
\noindent \textbf{Handling the Cold-start Problem.} Since \texttt{RL4Sugg} relies on feedback from annotators to capture search intentionality, there is a potential issue of a cold-start problem when recommending suggestions, especially when the learned knowledge may be insufficient for online user queries. To tackle this challenge, we employ an online learning strategy for \texttt{RL4Sugg}, continuously fine-tuning both the RewardNet and the PolicyNet using newly recorded query images and the suggestions clicked by users. This approach ensures that the model's policy remains up-to-date for online applications. In Section~\ref{sec:effectiveness}, we validate the effectiveness of this strategy, and the results demonstrate that the deployed system incorporating this approach significantly enhances the user experience. For example, we observe a remarkable increase in click behaviors by {\Comment 0.31\%}, indicating the positive impact of this strategy.

\label{sec:application}

==> related.tex <==
\section{RELATED WORK}
\label{sec:related}

\subsection{Query Suggestion}

Query suggestion is a feature of search engines that provides users with a list of possible queries based on their current query input. This can be helpful for users to explore their information need, and express their search intention more precisely. We review the literature in terms of Textual Query Suggestion (TQS) and Visual Query Suggestion (VQS). 

For TQS, it relies on the text of the user's query to generate a list of possible textual queries. There are a number of different methods for generating the query suggestions, including 
%
(i) query auto completion (it suggests queries based on the words that the user has typed)~\cite{shokouhi2013learning, bar2011context}, 
%
(ii) query spelling correction (it suggests queries that are spelled correctly)~\cite{hagen2017large,chen2007improving}, 
%
(iii) query expansion (it suggests queries that are related to the query that the user has typed)~\cite{carpineto2012survey, wen2001clustering}, and 
%
(iv) query rewriting (it suggests queries that are different from the query that the user has typed, but that are still relevant to the user's information need)~\cite{gottlob2014query,yu2004constraint,gottlob2011ontological}. Specifically, 
%
for (i),  Shokouhi et al.~\cite{shokouhi2013learning} propose a personalized Query Auto Completion (QAC) ranking system, which improves the accuracy and relevance of QAC suggestions for individual users, by considering the user's long-term search history and location.
%
For (ii), Hagen et al.~\cite{hagen2017large} create a large-scale corpus of queries with manually annotated spelling corrections, and it is further used to evaluate the spelling correction performance of existing commercial search systems.
%
For (iii), Cui et al.~\cite{cui2002probabilistic} propose a new query expansion method to improve search performance, by extracting probabilistic correlations between query terms and document terms through analyzing users' query logs. 
%
For (iv), Gottlob et al.~\cite{gottlob2011ontological} rewrite an ontological query into an equivalent query based on an underlying relational database, while a query optimization algorithm is proposed to improve the process more cost-effectively. Overall, TQS does not use any visual information, such as images, to generate suggestions. 

For VQS, it is introduced by Zha et al.~\cite{zha2009visual, zha2010visual}, which offers users both textual and visual suggestions based on their query text. This enables users to conveniently specify their search intentions. When a user selects a text-image pair from the suggestion list, the VQS system performs an image search using the provided text and employs the selected image to filter initial search results by leveraging its visual content. Subsequently, many techniques are proposed for the VQS. For example, 
%
Zeng et al.~\cite{zeng2017searching} develop a new client-side photo search system, which uses VQS and joint text-image hashing to improve the search accuracy and efficiency.
%
Li et al.~\cite{li2011mqss} study video search, and a multimodal method is developed to process the joint text and images suggestions produced by VQS. 
%
Overall, our MMQS problem differs from VQS mainly in that the user’s query input is different. In MMQS, the input is images, while in VQS, it is text. Additionally, Bian et al.~\cite{bian2012visual} study a new setting of VQS called Visual Query Attributes Suggestion (VQAS), where an image is inputted and VQAS suggests informative attributes (e.g., color, texture, shape) extracted from the query image via some SVM classifiers. These attributes allow users to select and express more precise search intents. Our work differs from VQAS in two aspects. First, MMQS outputs query suggestions instead of those image attributes, where the suggestions need satisfying the intentionality and diversity properties. Second, we propose a multi-agent reinforcement learning based framework to generate the suggestions from large language models instead of choosing those pre-defined attributes using classifiers.

\subsection{Vision-Language Pre-training}
Our work is related to Vision-Language Pre-training (VLP) in techniques. VLP aims to train a multimodal foundation model to align the relationships between images and text, and then the model is used to support various downstream vision-and-language tasks (e.g., image captioning or visual question answering). We review the literature of VLP in terms of different training strategies, i.e., (1) end-to-end pre-training, (2) modular pre-training, and (3) zero-shot.

For (1), it trains the whole multimodal model including image encoders and language models end-to-end, and different architectures are proposed for different tasks~\cite{li2023blip}, including the dual-encoder architecture~\cite{radford2021learning, jia2021scaling}, the fusion-encoder architecture~\cite{tan2019lxmert,li2021align}, the encoder-decoder architecture~\cite{cho2021unifying, wang2021simvlm}, and the unified transformer architecture~\cite{li2022blip,wang2023image,huang2023language}. For example,
%
Kosmos-1~\cite{huang2023language} is trained from scratch on multimodal Web corpora, including text, images, and image-caption pairs, and its training objective is based on next-token prediction task (e.g., image captioning), where it learns to generate the subsequent tokens based on the preceding tokens. In general, the majority of VLP models employed end-to-end pre-training need extensive image-text paired datasets, and as the model size increases, the pre-training process becomes computationally expensive.

For (2), it makes use of off-the-shelf pre-trained models, keeping them frozen during the pre-training. Existing studies can be categorized according to different frozen components, including the approaches that freeze image encoders~\cite{zhai2022lit,zhang2021vinvl}, language models~\cite{driess2023palm,guo2022images,chen2022visualgpt}, and both~\cite{li2023blip, alayrac2022flamingo,liu2023visual}. Specifically, 
%
Zhai et al.~\cite{zhai2022lit} study Locked-image Tuning (LiT), where it fine-tunes language models via contrastive learning to extract useful representations from locked pre-trained image models for new vision tasks.
%
Driess et al.~\cite{driess2023palm} propose embodied language models, which integrate visual information through a projector into language models. It freezes the language model, and just trains the image encoder with the projector for robotics tasks.
%
Flamingo~\cite{alayrac2022flamingo} freezes both image encoders and language models, and introduces cross-attention layers into the language model to incorporate visual features during the fine-tuning.
%
Similarly, BLIP-2~\cite{li2023blip} introduces an adapter called Q-Former, which injects visual features into the language model. Our \texttt{RL4Sugg} falls into this category of freezing both image encoders and language models, where we introduce a lightweight transformer-based module for fine-tuning, which aligns the input image to generate query suggestions with RLHF.

For (3), some recent works are proposed to enable some powerful large language models (e.g., ChatGPT) to solve vision-language tasks without training (i.e., zero-shot). For example, Visual ChatGPT~\cite{wu2023visual} constructs a pool of Visual Foundation Models (VFMs) such as image caption models or object detection models, and it designs a set of prompts that guide ChatGPT to call VFMs to finish various vision tasks. Then, different studies are proposed for different VFMs constructions (e.g., HuggingGPT~\cite{shen2023hugginggpt}) or prompts (e.g., MM-REACT~\cite{yang2023mm}).

\subsection{Reinforcement Learning from Human Feedback}
Reinforcement Learning from Human Feedback (RLHF) is an active research area that focuses on training RL agents using human-generated feedback, which is originally developed for training simple robots to interact with real-world environments for complex tasks such as Atari games~\cite{christiano2017deep}. 
%
Recently, RLHF has been applied to fine-tune various language tasks including text summarization~\cite{wu2021recursively,stiennon2020learning}, dialogue systems~\cite{jaques2019way,yi2019towards}, machine translation~\cite{kreutzer2018can,bahdanau2016actor}, semantic parsing~\cite{lawrence2018improving}, and review generation~\cite{cho2018towards}. For example, InstructGPT~\cite{ouyang2022training} collects a dataset of model desired outputs written by human labelers, and it then adopts RLHF to fine-tune GPT-3~\cite{brown2020language}.
%
In this paper, we propose a novel multi-agent reinforcement learning framework, which incorporates RLHF to generate human intentional query suggestions. To our best knowledge, this is the first of its kind.
